Robust Forecasting for Robotic Control: A Game-Theoretic Approach

Modern robots require accurate forecasts to make optimal decisions in the real world. For example, self-driving cars need an accurate forecast of other agents' future actions to plan safe trajectories. Current methods rely heavily on historical time series to accurately predict the future. However, relying entirely on the observed history is problematic since it could be corrupted by noise, have outliers, or not completely represent all possible outcomes. To solve this problem, we propose a novel framework for generating robust forecasts for robotic control. In order to model real-world factors affecting future forecasts, we introduce the notion of an adversary, which perturbs observed historical time series to increase a robot's ultimate control cost. Specifically, we model this interaction as a zero-sum two-player game between a robot's forecaster and this hypothetical adversary. We show that our proposed game may be solved to a local Nash equilibrium using gradient-based optimization techniques. Furthermore, we show that a forecaster trained with our method performs 30.14% better on out-of-distribution real-world lane change data than baselines.

==> figures_latex/arch.tex <==
\begin{figure}[t]
    \includegraphics[width=\columnwidth]{images/game_adver.png}
\vspace{-0.5em}
\caption{\small{ \textbf{Architecture:} We show the robotic system's architecture consisting of the forecaster, adversary and the controller. Nominally, the forecaster observes historical time series, $\history$, and predicts the future trajectory, $\futurepred$. The controller, $\pi$, generates the control signal, $\hat{u}$ and the control cost associated with it $J^c$. In order to model the real-world factors affecting the decision making of the forecaster, we introduce an adversary, $\adversary$, which perturbs the observed historical time series to an adversarial time series $
\historyadv$. As such, the adversary generates perturbations which maximize the control cost, while the forecaster generates future forecasts which minimize the control cost.}}
\label{fig:arch}
\end{figure}

